Joint H.E.S.S. and Fermi-LAT analysis of the region around PSR J1813-1749

HESS J1813-178 is one of the brightest sources detected during the first HESS Galactic Plane survey. The compact source, also detected by MAGIC, is believed to be a pulsar wind nebula powered by one of the most powerful pulsars known in the Galaxy, PSR J1813-1749 with a spin-down luminosity of $\dot{\mathrm{E}} = 5.6 \cdot 10^{37}\,\mathrm{erg}\,\mathrm{s}^{-1}$. With its extreme physical properties, as well as the pulsar's young age of 5.6 kyrs, the $\gamma$-rays detected in this region allow us to study the evolution of a highly atypical system. Previous studies of the region in the GeV energy range show emission extended beyond the size of the compact H.E.S.S. source. Using the archival H.E.S.S. data with improved background methods, we perform a detailed morphological and spectral analysis of the region. Additionally to the compact, bright emission component, we find significantly extended emission, whose position is coincident with HESS J1813-178. We reanalyse the region in GeV and derive a joint-model in order to find a continuous description of the emission in the region from GeV to TeV. Using the results derived in this analysis, as well as X-ray and radio data of the region, we perform multi-wavelength spectral modeling. Possible hadronic or leptonic origins of the $\gamma$-ray emission are investigated, and the diffusion parameters necessary to explain the extended emission are examined.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".


==> authors_ALL_ICRC2023.tex <==
\scriptsize
\noindent
F.~Aharonian$^{1,2,3}$, 
F.~Ait~Benkhali$^{4}$, 
A.~Alkan$^{5}$, 
J.~Aschersleben$^{6}$, 
H.~Ashkar$^{7}$, 
M.~Backes$^{8,9}$, 
A.~Baktash$^{10}$, 
V.~Barbosa~Martins$^{11}$, 
A.~Barnacka$^{12}$, 
J.~Barnard$^{13}$, 
R.~Batzofin$^{14}$, 
Y.~Becherini$^{15,16}$, 
G.~Beck$^{17}$, 
D.~Berge$^{11,18}$, 
K.~Bernl\"ohr$^{2}$, 
B.~Bi$^{19}$, 
M.~B\"ottcher$^{9}$, 
C.~Boisson$^{20}$, 
J.~Bolmont$^{21}$, 
M.~de~Bony~de~Lavergne$^{5}$, 
J.~Borowska$^{18}$, 
M.~Bouyahiaoui$^{2}$, 
F.~Bradascio$^{5}$, 
M.~Breuhaus$^{2}$, 
R.~Brose$^{1}$, 
A.~Brown$^{22}$, 
F.~Brun$^{5}$, 
B.~Bruno$^{23}$, 
T.~Bulik$^{24}$, 
C.~Burger-Scheidlin$^{1}$, 
T.~Bylund$^{5}$, 
F.~Cangemi$^{21}$, 
S.~Caroff$^{25}$, 
S.~Casanova$^{26}$, 
R.~Cecil$^{10}$, 
J.~Celic$^{23}$, 
M.~Cerruti$^{15}$, 
P.~Chambery$^{27}$, 
T.~Chand$^{9}$, 
S.~Chandra$^{9}$, 
A.~Chen$^{17}$, 
J.~Chibueze$^{9}$, 
O.~Chibueze$^{9}$, 
T.~Collins$^{28}$, 
G.~Cotter$^{22}$, 
P.~Cristofari$^{20}$, 
J.~Damascene~Mbarubucyeye$^{11}$, 
I.D.~Davids$^{8}$, 
J.~Davies$^{22}$, 
L.~de~Jonge$^{9}$, 
J.~Devin$^{29}$, 
A.~Djannati-Ata\"i$^{15}$, 
A.~Dmytriiev$^{9}$, 
V.~Doroshenko$^{19}$, 
L.~Dreyer$^{9}$, 
L.~Du~Plessis$^{9}$, 
K.~Egberts$^{14}$, 
S.~Einecke$^{28}$, 
J.-P.~Ernenwein$^{30}$, 
S.~Fegan$^{7}$, 
K.~Feijen$^{15}$, 
G.~Fichet~de~Clairfontaine$^{20}$, 
G.~Fontaine$^{7}$, 
F.~Lott$^{8}$, 
M.~F\"u{\ss}ling$^{11}$, 
S.~Funk$^{23}$, 
S.~Gabici$^{15}$, 
Y.A.~Gallant$^{29}$, 
S.~Ghafourizadeh$^{4}$, 
G.~Giavitto$^{11}$, 
L.~Giunti$^{15,5}$, 
D.~Glawion$^{23}$, 
J.F.~Glicenstein$^{5}$, 
J.~Glombitza$^{23}$, 
P.~Goswami$^{15}$, 
G.~Grolleron$^{21}$, 
M.-H.~Grondin$^{27}$, 
L.~Haerer$^{2}$, 
S.~Hattingh$^{9}$, 
M.~Haupt$^{11}$, 
G.~Hermann$^{2}$, 
J.A.~Hinton$^{2}$, 
W.~Hofmann$^{2}$, 
T.~L.~Holch$^{11}$, 
M.~Holler$^{31}$, 
D.~Horns$^{10}$, 
Zhiqiu~Huang$^{2}$, 
A.~Jaitly$^{11}$, 
M.~Jamrozy$^{12}$, 
F.~Jankowsky$^{4}$, 
A.~Jardin-Blicq$^{27}$, 
V.~Joshi$^{23}$, 
I.~Jung-Richardt$^{23}$, 
E.~Kasai$^{8}$, 
K.~Katarzy{\'n}ski$^{32}$, 
H.~Katjaita$^{8}$, 
D.~Khangulyan$^{33}$, 
R.~Khatoon$^{9}$, 
B.~Kh\'elifi$^{15}$, 
S.~Klepser$^{11}$, 
W.~Klu\'{z}niak$^{34}$, 
Nu.~Komin$^{17}$, 
R.~Konno$^{11}$, 
K.~Kosack$^{5}$, 
D.~Kostunin$^{11}$, 
A.~Kundu$^{9}$, 
G.~Lamanna$^{25}$, 
R.G.~Lang$^{23}$, 
S.~Le~Stum$^{30}$, 
V.~Lefranc$^{5}$, 
F.~Leitl$^{23}$, 
A.~Lemi\`ere$^{15}$, 
M.~Lemoine-Goumard$^{27}$, 
J.-P.~Lenain$^{21}$, 
F.~Leuschner$^{19}$, 
A.~Luashvili$^{20}$, 
I.~Lypova$^{4}$, 
J.~Mackey$^{1}$, 
D.~Malyshev$^{19}$, 
D.~Malyshev$^{23}$, 
V.~Marandon$^{5}$, 
A.~Marcowith$^{29}$, 
P.~Marinos$^{28}$, 
G.~Mart\'i-Devesa$^{31}$, 
R.~Marx$^{4}$, 
G.~Maurin$^{25}$, 
A.~Mehta$^{11}$, 
P.J.~Meintjes$^{13}$, 
M.~Meyer$^{10}$, 
A.~Mitchell$^{23}$, 
R.~Moderski$^{34}$, 
L.~Mohrmann$^{2}$, 
A.~Montanari$^{4}$, 
C.~Moore$^{35}$, 
E.~Moulin$^{5}$, 
T.~Murach$^{11}$, 
K.~Nakashima$^{23}$, 
M.~de~Naurois$^{7}$, 
H.~Ndiyavala$^{8,9}$, 
J.~Niemiec$^{26}$, 
A.~Priyana~Noel$^{12}$, 
P.~O'Brien$^{35}$, 
S.~Ohm$^{11}$, 
L.~Olivera-Nieto$^{2}$, 
E.~de~Ona~Wilhelmi$^{11}$, 
M.~Ostrowski$^{12}$, 
E.~Oukacha$^{15}$, 
S.~Panny$^{31}$, 
M.~Panter$^{2}$, 
R.D.~Parsons$^{18}$, 
U.~Pensec$^{21}$, 
G.~Peron$^{15}$, 
S.~Pita$^{15}$, 
V.~Poireau$^{25}$, 
D.A.~Prokhorov$^{36}$, 
H.~Prokoph$^{11}$, 
G.~P\"uhlhofer$^{19}$, 
M.~Punch$^{15}$, 
A.~Quirrenbach$^{4}$, 
M.~Regeard$^{15}$, 
P.~Reichherzer$^{5}$, 
A.~Reimer$^{31}$, 
O.~Reimer$^{31}$, 
I.~Reis$^{5}$, 
Q.~Remy$^{2}$, 
H.~Ren$^{2}$, 
M.~Renaud$^{29}$, 
B.~Reville$^{2}$, 
F.~Rieger$^{2}$, 
G.~Roellinghoff$^{23}$, 
E.~Rol$^{36}$, 
G.~Rowell$^{28}$, 
B.~Rudak$^{34}$, 
H.~Rueda Ricarte$^{5}$, 
E.~Ruiz-Velasco$^{2}$, 
K.~Sabri$^{29}$, 
V.~Sahakian$^{3}$, 
S.~Sailer$^{2}$, 
H.~Salzmann$^{19}$, 
D.A.~Sanchez$^{25}$, 
A.~Santangelo$^{19}$, 
M.~Sasaki$^{23}$, 
J.~Sch\"afer$^{23}$, 
F.~Sch\"ussler$^{5}$, 
H.M.~Schutte$^{9}$, 
M.~Senniappan$^{16}$, 
J.N.S.~Shapopi$^{8}$, 
S.~Shilunga$^{8}$, 
K.~Shiningayamwe$^{8}$, 
H.~Sol$^{20}$, 
H.~Spackman$^{22}$, 
A.~Specovius$^{23}$, 
S.~Spencer$^{23}$, 
{\L.}~Stawarz$^{12}$, 
R.~Steenkamp$^{8}$, 
C.~Stegmann$^{14,11}$, 
S.~Steinmassl$^{2}$, 
C.~Steppa$^{14}$, 
K.~Streil$^{23}$, 
I.~Sushch$^{9}$, 
H.~Suzuki$^{37}$, 
T.~Takahashi$^{38}$, 
T.~Tanaka$^{37}$, 
T.~Tavernier$^{5}$, 
A.M.~Taylor$^{11}$, 
R.~Terrier$^{15}$, 
A.~Thakur$^{28}$, 
J.~H.E.~Thiersen$^{9}$, 
C.~Thorpe-Morgan$^{19}$, 
M.~Tluczykont$^{10}$, 
M.~Tsirou$^{11}$, 
N.~Tsuji$^{39}$, 
R.~Tuffs$^{2}$, 
Y.~Uchiyama$^{33}$, 
M.~Ullmo$^{5}$, 
T.~Unbehaun$^{23}$, 
P.~van~der~Merwe$^{9}$, 
C.~van~Eldik$^{23}$, 
B.~van~Soelen$^{13}$, 
G.~Vasileiadis$^{29}$, 
M.~Vecchi$^{6}$, 
J.~Veh$^{23}$, 
C.~Venter$^{9}$, 
J.~Vink$^{36}$, 
H.J.~V\"olk$^{2}$, 
N.~Vogel$^{23}$, 
T.~Wach$^{23}$, 
S.J.~Wagner$^{4}$, 
F.~Werner$^{2}$, 
R.~White$^{2}$, 
A.~Wierzcholska$^{26}$, 
Yu~Wun~Wong$^{23}$, 
H.~Yassin$^{9}$, 
M.~Zacharias$^{4,9}$, 
D.~Zargaryan$^{1}$, 
A.A.~Zdziarski$^{34}$, 
A.~Zech$^{20}$, 
S.J.~Zhu$^{11}$, 
A.~Zmija$^{23}$, 
S.~Zouari$^{15}$ and 
N.~\.Zywucka$^{9}$.

\medskip


\noindent
$^{1}$Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, Dublin 2, Ireland\\
$^{2}$Max-Planck-Institut f\"ur Kernphysik, P.O. Box 103980, D 69029 Heidelberg, Germany\\
$^{3}$Yerevan State University,  1 Alek Manukyan St, Yerevan 0025, Armenia\\
$^{4}$Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany\\
$^{5}$IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France\\
$^{6}$Kapteyn Astronomical Institute, University of Groningen, Landleven 12, 9747 AD Groningen, The Netherlands\\
$^{7}$Laboratoire Leprince-Ringuet, École Polytechnique, CNRS, Institut Polytechnique de Paris, F-91128 Palaiseau, France\\
$^{8}$University of Namibia, Department of Physics, Private Bag 13301, Windhoek 10005, Namibia\\
$^{9}$Centre for Space Research, North-West University, Potchefstroom 2520, South Africa\\
$^{10}$Universit\"at Hamburg, Institut f\"ur Experimentalphysik, Luruper Chaussee 149, D 22761 Hamburg, Germany\\
$^{11}$DESY, D-15738 Zeuthen, Germany\\
$^{12}$Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, ul. Orla 171, 30-244 Krak{\'o}w, Poland\\
$^{13}$Department of Physics, University of the Free State,  PO Box 339, Bloemfontein 9300, South Africa\\
$^{14}$Institut f\"ur Physik und Astronomie, Universit\"at Potsdam,  Karl-Liebknecht-Strasse 24/25, D 14476 Potsdam, Germany\\
$^{15}$Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France\\
$^{16}$Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden\\
$^{17}$School of Physics, University of the Witwatersrand, 1 Jan Smuts Avenue, Braamfontein, Johannesburg, 2050 South Africa\\
$^{18}$Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, Newtonstr. 15, D 12489 Berlin, Germany\\
$^{19}$Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, D 72076 T\"ubingen, Germany\\
$^{20}$Laboratoire Univers et Théories, Observatoire de Paris, Université PSL, CNRS, Université de Paris, 92190 Meudon, France\\
$^{21}$Sorbonne Universit\'e, Universit\'e Paris Diderot, Sorbonne Paris Cit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies, LPNHE, 4 Place Jussieu, F-75252 Paris, France\\
$^{22}$University of Oxford, Department of Physics, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK\\
$^{23}$Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Nikolaus-Fiebiger-Str. 2, D 91058 Erlangen, Germany\\
$^{24}$Astronomical Observatory, The University of Warsaw, Al. Ujazdowskie 4, 00-478 Warsaw, Poland\\
$^{25}$Université Savoie Mont Blanc, CNRS, Laboratoire d'Annecy de Physique des Particules - IN2P3, 74000 Annecy, France\\
$^{26}$Instytut Fizyki J\c{a}drowej PAN, ul. Radzikowskiego 152, 31-342 Krak{\'o}w, Poland\\
$^{27}$Universit\'e Bordeaux, CNRS, LP2I Bordeaux, UMR 5797, F-33170 Gradignan, France\\
$^{28}$School of Physical Sciences, University of Adelaide, Adelaide 5005, Australia\\
$^{29}$Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, CNRS/IN2P3,  CC 72, Place Eug\`ene Bataillon, F-34095 Montpellier Cedex 5, France\\
$^{30}$Aix Marseille Universit\'e, CNRS/IN2P3, CPPM, Marseille, France\\
$^{31}$Leopold-Franzens-Universit\"at Innsbruck, Institut f\"ur Astro- und Teilchenphysik, A-6020 Innsbruck, Austria\\
$^{32}$Institute of Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University,  Grudziadzka 5, 87-100 Torun, Poland\\
$^{33}$Department of Physics, Rikkyo University, 3-34-1 Nishi-Ikebukuro, Toshima-ku, Tokyo 171-8501, Japan\\
$^{34}$Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, ul. Bartycka 18, 00-716 Warsaw, Poland\\
$^{35}$Department of Physics and Astronomy, The University of Leicester, University Road, Leicester, LE1 7RH, United Kingdom\\
$^{36}$GRAPPA, Anton Pannekoek Institute for Astronomy, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands\\
$^{37}$Department of Physics, Konan University, 8-9-1 Okamoto, Higashinada, Kobe, Hyogo 658-8501, Japan\\
$^{38}$Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study (UTIAS), The University of Tokyo, 5-1-5 Kashiwa-no-Ha, Kashiwa, Chiba, 277-8583, Japan\\
$^{39}$RIKEN, 2-1 Hirosawa, Wako, Saitama 351-0198, Japan\\

